Balancing Morality and Economics: Population Games with Herding and Inertia

The adoption of clean technologies (CTs) plays an important role in reducing carbon dioxide (CO$_2$) emissions. We study CT adoption in a large population of consumers with heterogeneous behavioral tendencies. We model the interaction among the agents as a multi-type mean-field game in which the agents choose between clean and polluting technology based products and may either behave as rationals (trading off price and moral incentives), herding agents (just follow the majority), or lethargic agents exhibiting inertia toward adopting the new technologies. We characterize equilibrium CT adoption levels using the recently introduced notion of $\boldsymbol{\alpha}$-Rational Nash Equilibrium ($\boldsymbol{\alpha}$-RNE) and its multi-type extension. We then identify a stable subset using the limits of a stochastic turn-by-turn behavioral dynamics. Our results highlight the role of population composition in determining CT adoption. In particular, widespread adoption requires either a sufficiently small price disadvantage for CTs or the presence of a sufficiently large herding population that can be influenced through social awareness programs. Surprisingly, we could prove that environmental damages do not provide sufficient incentives to increase CT adoption.

==> dynamic.tex <==
\section{Dynamic Stability and Equilibrium Selection}
\label{sec:dyn}
In this section, we study which $\alpha$-RNE equilibria are selected under a
natural population adjustment process. While Section~II characterizes the
complete set $\mathcal N_\alpha$ of $\alpha$-RNEs, not all equilibria are
dynamically relevant. We show that, under standard evolutionary dynamics, the
population converges to stable equilibria, thereby providing an equilibrium
selection mechanism.

\subsection{Replicator Dynamics}
We consider a continuous-time adjustment process in which the fraction $z(t)$ of
agents adopting the clean technology evolves according to the replicator
dynamics
\begin{equation}\label{eq:replicator}
\dot z(t)= z(t)\bigl(1-z(t)\bigr)\,h\bigl(z(t)\bigr),
\end{equation}
where the utility difference function $h(\cdot)$ is defined from
\eqref{eqn_utility_players1} as
\begin{equation}\label{eq:h_dyn}
h(z):=u(1,z)-u(2,z)=P_{uc}-P_c+2(1-z)z\,u_m
= -\Delta_P +2(1-z)z\,u_m .
\end{equation}
Dynamics of the form \eqref{eq:replicator} arise naturally in evolutionary game
theory and model payoff-based learning and imitation in large populations
\cite{hofbauer1998evolutionary}. Moreover, the unit interval is forward
invariant: if $z(0)\in[0,1]$, then $z(t)\in[0,1]$ for all $t\ge 0$.
\subsection{Stationary Points}
A stationary point $z^*$ of \eqref{eq:replicator} satisfies
$$
z^*(1-z^*)h(z^*)=0.
$$
Hence, stationary points are given by
$$
z^* \in \{0,1\}\cup\{z\in(0,1):h(z)=0\}.
$$
When $\Delta_P<\nicefrac{u_m}{2}$, the equation $h(z)=0$ admits two interior solutions
\begin{equation}\label{eq:roots_dyn}
R^+ := \frac{1+\sqrt{1-2\Delta_P/u_m}}{2},\qquad
R^- := \frac{1-\sqrt{1-2\Delta_P/u_m}}{2}.
\end{equation}
Otherwise, no interior stationary point exists.

\subsection{Local Stability}
We next characterize the local stability of the stationary points of
\eqref{eq:replicator}.
\begin{theorem}\label{thm:stability}
Consider the replicator dynamics \eqref{eq:replicator}.
\begin{enumerate}
\item If $\Delta_P \ge \nicefrac{u_m}{2}$, then $z=0$ is globally asymptotically stable in $(0,1)$.
\item If $\Delta_P<u_m/2$, then:
\begin{itemize}
\item $R^-$ is locally asymptotically stable;
\item $R^+$ is unstable;
\item $z=0$ and $z=1$ are unstable.
\end{itemize}
\end{enumerate}
\end{theorem}

\begin{proof}
Let $F(z):=z(1-z)h(z)$, so that $\dot z=F(z)$.
Local stability is determined by the sign of $F'(z^*)$.

From \eqref{eq:h_dyn}, we have $h'(z)=2u_m(1-2z)$, and hence
$$
F'(z)=(1-2z)h(z)+z(1-z)h'(z).
$$
\emph{Case 1: $\Delta_P\ge u_m/2$.}
Then $h(z)<0$ for all $z\in(0,1)$, so $F(z)<0$ on $(0,1)$ and thus $z(t)$
decreases monotonically to $0$ for any $z(0)\in(0,1)$.

\emph{Case 2: $\Delta_P<u_m/2$.}
Then $h(R^-)=h(R^+)=0$, with $h(z)>0$ on $(R^-,R^+)$ and $h(z)<0$ on
$(0,R^-)\cup(R^+,1)$.
Evaluating $F'$ at $R^-$ and $R^+$ gives
$$
F'(R^-)=R^-(1-R^-)h'(R^-)<0,
F'(R^+)=R^+(1-R^+)h'(R^+)>0,
$$
since $h'(R^-)<0$ and $h'(R^+)>0$. Hence $R^-$ is locally asymptotically stable
and $R^+$ is unstable. Finally, $F'(0)=h(0)<0$ and $F'(1)=h(1)<0$, implying that
both boundary equilibria are unstable.
\end{proof}

\subsection{Equilibrium Selection and Relation to $\alpha$-RNE}

We now describe the convergence behavior of \eqref{eq:replicator} and relate the
limit points to the $\alpha$-RNE set $\mathcal N_\alpha$ characterized in
Section~II.

\begin{theorem}\label{thm:selection}
Assume $\Delta_P<u_m/2$ and let $z(t)$ be a solution of \eqref{eq:replicator}
with $z(0)\in(0,1)$. Then:
\begin{enumerate}
\item if $z(0)\in(0,R^-)$, then $z(t)\to 0$;
\item if $z(0)\in(R^-,R^+)$, then $z(t)\to R^-$;
\item if $z(0)\in(R^+,1)$, then $z(t)\to 1$.
\end{enumerate}
In particular, among the stationary points of \eqref{eq:replicator}, only the
dynamically stable ones are relevant for long-run outcomes; the corresponding
equilibrium outcome must additionally lie in $\mathcal N_\alpha$.
\end{theorem}
\begin{proof}
The sign structure of $F(z)=z(1-z)h(z)$ implies $\dot z>0$ on $(R^-,R^+)$ and
$\dot z<0$ on $(0,R^-)\cup(R^+,1)$. Standard phase-line arguments for scalar
autonomous systems imply convergence to the attracting stationary point in each
interval, yielding the stated limits. The final statement follows because
$\alpha$-RNE imposes admissibility conditions on equilibrium outcomes, as
characterized in Section~II.
\end{proof}
\subsection{Implications for Herding Behavior}
Theorems~\ref{thm:stability}--\ref{thm:selection} show that, although multiple
$\alpha$-RNEs may exist, only dynamically stable equilibria are selected under
payoff-based learning. In particular, the unstable equilibrium $R^+$ is never
observed in the long run, justifying its exclusion from the comparison of
equilibrium adoption outcomes.

